Abstraction-driven Concolic Testing

Concolic testing is a promising method for generating test suites for large programs. However, it suffers from the path-explosion problem and often fails to find tests that cover difficult-to-reach parts of programs. In contrast, model checkers based on counterexample-guided abstraction refinement explore programs exhaustively, while failing to scale on large programs with precision. In this paper, we present a novel method that iteratively combines concolic testing and model checking to find a test suite for a given coverage criterion. If concolic testing fails to cover some test goals, then the model checker refines its program abstraction to prove more paths infeasible, which reduces the search space for concolic testing. We have implemented our method on top of the concolic-testing tool CREST and the model checker CpaChecker. We evaluated our tool on a collection of programs and a category of SvComp benchmarks. In our experiments, we observed an improvement in branch coverage compared to CREST from 48% to 63% in the best case, and from 66% to 71% on average.

==> abstract-archiv.tex <==
Concolic testing is a promising method for generating test suites 
for large programs.
However, it suffers from the path-explosion problem and often fails to 
find tests that cover difficult-to-reach parts of programs.
In contrast, model checkers based on counterexample-guided abstraction
refinement explore programs exhaustively, while failing to scale on 
large programs with precision.
In this paper, we present a novel method that iteratively combines concolic 
testing and model checking to find a test suite for a given coverage criterion.
If concolic testing fails to cover some test goals, then the model checker 
refines its program abstraction to prove more paths infeasible, which reduces 
the search space for concolic testing.
We have implemented our method on top of the concolic-testing tool CREST and 
the model checker CpaChecker.
We evaluated our tool on a collection of programs and a category of SvComp benchmarks.
In our experiments, we observed an improvement in branch coverage compared to CREST
from 48% to 63% in the best case, and from 66% to 71% on average.



==> cbmc.tex <==
\section{Example - CBMC}
First we motivate our approach on a CBMC example.
The program in \ref{fig:cbmc1} contains a loop that is executed 10000 times and a branch inside the loop.
To check if the assertion is violated, CBMC constructs a long SMT formula with many disjunctions that arise from the branching.
It takes 19sec for CBMC to check that the assertion holds.

\begin{figure}[h]
  \centering
\begin{lstlisting}
 const int N=10000;
  int x=1;

  for (int i=0; i<N; i++){    
    if (x > 0)
    x++;
    else
    x = -x + 1;
  }
  assert(x > 2000);
\end{lstlisting}
  \caption{Program with a branching inside a loop.}
\label{fig:cbmc1}
\end{figure}


By inspecting the program, we see that the ``else'' branch is never executed.
We simplify the program, we syntactically removing the spurious branch -- this operation is equivalent to refining the CFG.
The refined program is shown in Figure \ref{fig:cbmc2}.
Now, CBMC needs only 1sec to check that the assertion holds, because it doesn't construct SMT constrains for infeasible behaviors in the CFG.


\begin{figure}[h]
  \centering
\begin{lstlisting}
 const int N=10000;
  int x=1;

  for (int i=0; i<N; i++){
    x++;
  }
  assert(x > 2000);
\end{lstlisting}
  \caption{A refined program.}
\label{fig:cbmc2}
\end{figure}


==> concolic-example.tex <==
% \section{Example - concolic testing}

% There are many heuristics to guide the way concolic testing explores the program.
% For instance, the ``static path'' heuristics  drives the search along the shortest path in the CFG from the current execution to some uncovered branch.

% However,  looking for the shortest path in the CFG can be misleading, because it may be infeasible.
% The program in Figure \ref{fig:con1} has $N$ independent branches and a special ``goal'' branch. 
% To cover the goal branch the first four branches need to be taken in the right order.

% If the goal branch hasn't been covered, then the static path heuristics will suggest to flip the bottom branches to hit the goal.
% This tactics is inefficient, because it's actually the first four branches than need to be flipped.
% For $N=12$ concolic testing needs on average 2573 iteration to cover the goal branch.


\begin{figure}[h]
  \centering
\begin{lstlisting}
  bool b0, ..., bN;

  // level 0
  if (input() > 0)
    b0 = 1;
  else 
    b0 = 0;

 ...

  // level N;
  if (input() > 0)
    bN = 1;
  else 
    bN = 0;
  
  if (!b0 && b1 && !b2 && b3){
    printf("Goal\n"); // special branch
  }
\end{lstlisting}
  \caption{Program with N independent branches.}
\label{fig:con1}
\end{figure}


% Now, suppose we refine the CFG by adding a check after the first four branches if the goal branch can be still reached.
% If the four branches are in the right order, then we proceed normally and otherwise we to go a copy of the program where the goal branch is missing.
% For the refined program, concolic testing needs only 19 iterations to cover the goal, as opposed to 2573 iterations in the original version.

\begin{figure}[h]
  \centering
  \scalebox{1}{\input{figures/cfg-conc}}
  \caption{CFG for the program in Figure \ref{fig:con1}. Suppose that the only goal to cover is location ``G''. Concolic testing uses shortest path heuristics to find the next symbolic path.}
  \label{fig:spec_alt}
\end{figure}


\begin{figure}[h]
  \centering
  \scalebox{1}{\input{figures/abs1}}
  \caption{Model checker runs on the CFG with the ``G'' target. It discovers predicate $b0$ and refines the abstraction before it times out. The figure show the abstraction, which becomes the monitor $\mathcal{M}$.}
  \label{fig:abs1}
\end{figure}




\begin{figure}[h]
  \centering
  \scalebox{1}{\input{figures/ref1}}
  \caption{Figure show product $P'$ of the program in Figure \ref{fig:con1} with the abstraction in Figure \ref{fig:abs1}. Concolic testing continues on $P'$. In $P'$ concolic testing know to backtrack to the first branch in order to reach the goal. }
  \label{fig:spec_alt}
\end{figure}






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> figures/cov_plot_ddvallfalse.tex <==
\begin{figure}[th]
  \begin{center}
    \input{graph2}
    \caption{Test coverage vs.  testing/model checkig ratio}
    \label{fig:cov_plot_ddvallfalse}
  \end{center}
\end{figure}

==> figures/graph1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4320.00,3024.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{}48%}}%
      \put(814,932){\makebox(0,0)[r]{\strut{}50%}}%
      \put(814,1161){\makebox(0,0)[r]{\strut{}52%}}%
      \put(814,1389){\makebox(0,0)[r]{\strut{}54%}}%
      \put(814,1617){\makebox(0,0)[r]{\strut{}56%}}%
      \put(814,1846){\makebox(0,0)[r]{\strut{}58%}}%
      \put(814,2074){\makebox(0,0)[r]{\strut{}60%}}%
      \put(814,2302){\makebox(0,0)[r]{\strut{}62%}}%
      \put(814,2531){\makebox(0,0)[r]{\strut{}64%}}%
      \put(814,2759){\makebox(0,0)[r]{\strut{}66%}}%
      \put(946,484){\makebox(0,0){\strut{} 0%}}%
      \put(1244,484){\makebox(0,0){\strut{}10%}}%
      \put(1541,484){\makebox(0,0){\strut{}20%}}%
      \put(1839,484){\makebox(0,0){\strut{}30%}}%
      \put(2137,484){\makebox(0,0){\strut{}40%}}%
      \put(2435,484){\makebox(0,0){\strut{}50%}}%
      \put(2732,484){\makebox(0,0){\strut{}60%}}%
      \put(3030,484){\makebox(0,0){\strut{}70%}}%
      \put(3328,484){\makebox(0,0){\strut{}80%}}%
      \put(3625,484){\makebox(0,0){\strut{}90%}}%
      \put(3923,484){\makebox(0,0){\strut{}100%}}%
      \put(176,1731){\rotatebox{-270}{\makebox(0,0){\strut{}Coverage}}}%
      \put(2434,154){\makebox(0,0){\strut{}testing/model checking}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graph1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot_nsi <==
set term epslatex
set output "graph1.eps"
set notitle 
set ylabel "Coverage"
set xlabel "$\frac{testing}{testing + model checking}$"
set format y '%2.0f%%'
set format x '%2.0f%%' 
set yrange [50:70]
# set xrange [0:100]
set size 0.45, 0.45
#set xtic auto                          # set xtics automatically
#set ytic auto                          # set ytics automatically
set ytics 10
set xtics 25
plot "../crabs/cpachecker/cov_nsi"  using 1:2 w linespoints ps 1 pt 7 notitle
